MADRL-based UAVs Trajectory Design with Anti-Collision Mechanism in Vehicular Networks

In upcoming 6G networks, unmanned aerial vehicles (UAVs) are expected to play a fundamental role by acting as mobile base stations, particularly for demanding vehicle-to-everything (V2X) applications. In this scenario, one of the most challenging problems is the design of trajectories for multiple UAVs, cooperatively serving the same area. Such joint trajectory design can be performed using multi-agent deep reinforcement learning (MADRL) algorithms, but ensuring collision-free paths among UAVs becomes a critical challenge. Traditional methods involve imposing high penalties during training to discourage unsafe conditions, but these can be proven to be ineffective, whereas binary masks can be used to restrict unsafe actions, but naively applying them to all agents can lead to suboptimal solutions and inefficiencies. To address these issues, we propose a rank-based binary masking approach. Higher-ranked UAVs move optimally, while lower-ranked UAVs use this information to define improved binary masks, reducing the number of unsafe actions. This approach allows to obtain a good trade-off between exploration and exploitation, resulting in enhanced training performance, while maintaining safety constraints.

==> Chapters/2_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
%\the\textwidth
Nowadays, the use of \acp{UAV} as flying \acp{BS}, namely \acp{UABS}, has gained considerable attention in the literature as a promising technology for future 6G networks \cite{EssayHentati,9815631}. The ability of \ac{UABS} to operate at high altitudes opens up the possibility of providing \ac{LoS} links with ground users, leading to enhanced network coverage and capacity for a wide variety of applications. An important use case is foreseen in vehicular communications~\cite{Extended_Sensing_1,white_paper}, where vehicles have to exchange large amounts of information with the network and among themselves. In such scenarios, \ac{UABS} can significantly enhance network performance.

Moreover, addressing complex urban environments poses a crucial challenge: the design of optimized trajectories for multiple \ac{UABS} to ensure a desired network performance. Additionally, introducing a coordination mechanism among \acp{UABS} becomes crucial to ensure optimal coverage of the environment while avoiding overlapping trajectories that may lead to interference or, even worse, flight collisions.

%%%%%% STATE OF THE ART %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Extensive research has been conducted on collision avoidance for \ac{UAV} swarms. Conventional methods include \ac{VO}, which involves frequent changes in \acp{UAV} velocities \cite{SnaBerGuy:J11}, \ac{APF}, which does not fully leverage drone cooperation \cite{HuaLow:C18}, and \ac{PSO}, which generates energy inefficient zigzag trajectories \cite{SonWanZou:J19}. 
Addressing these challenges often requires complex mathematical models and significant computational time. In response, machine learning-based solutions \cite{10095817, 9909656, marini2022continual}, particularly \ac{MADRL}-based algorithms \cite{TesFavGio:C20, GueGuiDar:J23}, offer promising alternative approaches to mitigate such issues.
Many existing works in the literature address collision avoidance by introducing constraints on the agents' mobility models and tweaking the reward function. These constraints enforce a minimum safety distance between any two agents at any time instant \cite{WanGur:J22,XuZhaLi:J22,ThuDeg:J22,QieShiShe:J19}. 
In these works, the reward function is modified to include a simple penalty term based on mutual distances between agents.
A slightly different approach is proposed in \cite{ThuDeg:J22}, where each agent is surrounded by a ‘repulsive field’ that induces negative and positive rewards proportional to encroachment and target distances, respectively.
Nevertheless, such methods restrict the movement space of agents, that are forced to learn sub-optimal policies. 
Furthermore, solutions like the ones proposed in the aforementioned works limit the collision probability but do not entirely prevent collisions, posing challenges when applied to real-world systems.
  
This paper presents a \ac{MADRL} model that can optimize the trajectories of a swarm of \ac{UABS} deployed over an urban scenario. The model is characterized by a mask-based mechanism that allows \ac{UABS} to avoid any flight collisions, as well as possible interference with other agents that are serving vehicular users under their fields of view. 
More specifically, to improve the agents' performance, a ranking system is introduced: high-ranked agents will have the opportunity to follow the best trajectories, whereas low ones will have to respect the safety constraint using binary masking. 
Results are presented in terms of the cumulative reward collected by agents, showing the convergence property of the training algorithm designed, and in terms of the percentage of satisfied users, indicating how well the proposed system can meet the stringent requirements of \ac{V2X} applications while respecting the safety constraint introduced. 

The rest of the paper is organized as follows: Section~\ref{sec:system_model} describes the system model, Section~\ref{sec:multi_agent} offers an overview of the \ac{MADRL} model and a detailed analysis of the proposed anti-collision mechanism, Section~\ref{sec:results} shows the results obtained and Section~\ref{sec:conclusion} depicts the main conclusions.
\newline
